Bad Values but Good Behavior: Learning Highly Misspecified Bandits and MDPs

Parametric, feature-based reward models are employed by a variety of algorithms in decision-making settings such as bandits and Markov decision processes (MDPs). The typical assumption under which the algorithms are analysed is realizability, i.e., that the true values of actions are perfectly explained by some parametric model in the class. We are, however, interested in the situation where the true values are (significantly) misspecified with respect to the model class. For parameterized bandits, contextual bandits and MDPs, we identify structural conditions, depending on the problem instance and model class, under which basic algorithms such as $\epsilon$-greedy, LinUCB and fitted Q-learning provably learn optimal policies under even highly misspecified models. This is in contrast to existing worst-case results for, say misspecified bandits, which show regret bounds that scale linearly with time, and shows that there can be a nontrivially large set of bandit instances that are robust to misspecification.

==> Contribution.tex <==
% \section{Contribution}

% Our main contribution is on an existential note. Most works in bandits till now have either resulted in a linear regret under the uniform model error assumption \citep{pmlr-v119-lattimore20a, zanette2020learning} or have modified the definition of misspecification to weaken the uniform notion of model errors \cite{pmlr-v216-liu23c}. Our target is a bit different. We focus on problems which can have a constant order model error, but simple algorithms like $\epsilon$-greedy are able to learn with zero regret. More precisely, we provide a sufficient condition on the parameterized class of function approximators and the true model class for which one is guaranteed to enjoy no regret despite having a constant order approximation error. We show that the $\epsilon$-greedy algorithm with a learning rate of $1/\sqrt{t}$ is able to get a regret order of $\mathcal{O}(\sqrt{T})$ on a large class of problems with a constant order approximation error. We extend our framework to the contextual bandits setting as well and analyze the $\epsilon$-greedy algorithm in this framework as well to show that with the $\epsilon$ tuned as $1\sqrt{t}$, one is able to get regret of the order of $\cO(\sqrt{T})$.


 

==> erratum.tex <==
\section{Errata}
We noticed that we had used a notation in the contextual bandit section \ref{subsec:Context} that first appeared in Theorem \ref{thm:context_sufficient}, which we have not defined formally. Though we believe that the notation is self-explanatory, we admit it was an overlook on our behalf. The notation in question is $\mathrm{OPT}(x)$ for a context $x$. This notation represents the optimal arm at context $x$. To be formally correct, we define 
\begin{align*}
    &\mathrm{OPT} : \Real^{\abs{\cA}} \to \cA \; \text{ as }\\
    &\mathrm{OPT}(\bm{\mu}) = \argmax_{a \in \cA} \mu_a\;,
\end{align*}
to represent the optimal arm for an $\abs{\cA}$ armed bandit problem.
Similarly for the contextual setting given any fixed context $x$ and it's corresponding context-specific reward vector $\bm{\mu_x}$, we have
\begin{align*}
    &\mathrm{OPT} : \Real^{\abs{\cA}} \to \cA \; \text{ as }\\
    &\mathrm{OPT}(\bm{\mu_x}) = \argmax_{a \in \cA} \mu_{x,a}\;.
\end{align*}
to denote the optimal arm at context $x$.
We abuse notation and write $\mathrm{OPT}(x)$ to denote $\mathrm{OPT}(\bm{\mu_x})$ as the optimal arm at context $x$.
